Similarity Learning for Authorship Verification in Social Media

Authorship verification tries to answer the question if two documents with unknown authors were written by the same author or not. A range of successful technical approaches has been proposed for this task, many of which are based on traditional linguistic features such as n-grams. These algorithms achieve good results for certain types of written documents like books and novels. Forensic authorship verification for social media, however, is a much more challenging task since messages tend to be relatively short, with a large variety of different genres and topics. At this point, traditional methods based on features like n-grams have had limited success. In this work, we propose a new neural network topology for similarity learning that significantly improves the performance on the author verification task with such challenging data sets.

==> simulation/plot.tex <==

\begin{figure}
\centering
\begin{tikzpicture}
\definecolor{mycolor1}{rgb}{0.803, 0.36, 0.36}%
\definecolor{mycolor2}{rgb}{0.274,0.509,0.705}%
\begin{axis}[
legend pos=north west,
legend style={font=\fontsize{7}{5}\selectfont},
enlargelimits={abs=0.5},
ybar=0pt,
bar width=0.4,
xtick={1, 2, 3, 4},
xlabel={},
xticklabels={Baseline, HRSN, pretr., data augm.},
ymin=67,
ymax=85,
axis background/.style={fill=white},
width=3.5in,
height=2in,
]

\addplot[fill=mycolor1, draw=black, area legend, error bars/.cd,
y dir=both,y explicit]
coordinates {
    (1,0.0) +- (0.0, 0.0)
    (2,82.0) +- (0.0, 1.1)
    (3,82.7) +- (0.0, 2.1)
    (4,83.0) +- (0.0, 1.0)};
\addplot[fill=mycolor2, draw=black, area legend, error bars/.cd,
y dir=both,y explicit]
coordinates {
    (1,69.9) +- (0.0, 1.7)
    (2,82.1) +- (0.0, 1.7)
    (3,82.1) +- (0.0, 1.1)
    (4,82.6) +- (0.0, 0.3)};
\legend{dev set, test set}
\end{axis}
\end{tikzpicture}
\end{figure}

